Relatedly: Scaffolding Literature Reviews with Existing Related Work Sections

Scholars who want to research a scientific topic must take time to read, extract meaning, and identify connections across many papers. As scientific literature grows, this becomes increasingly challenging. Meanwhile, authors summarize prior research in papers' related work sections, though this is scoped to support a single paper. A formative study found that while reading multiple related work paragraphs helps overview a topic, it is hard to navigate overlapping and diverging references and research foci. In this work, we design a system, Relatedly, that scaffolds exploring and reading multiple related work paragraphs on a topic, with features including dynamic re-ranking and highlighting to spotlight unexplored dissimilar information, auto-generated descriptive paragraph headings, and low-lighting of redundant information. From a within-subjects user study (n=15), we found that scholars generate more coherent, insightful, and comprehensive topic outlines using Relatedly compared to a baseline paper list.

==> 01_intro.tex <==
Scientific discovery and innovation rely upon scholars' rich understanding of prior work by reviewing the literature, but this process of extracting meaning, and identifying connections across many papers with large amounts of ambiguous domain-specific information \cite{knopf2006doing, zhang2008citesense} is getting progressively harder with the exponential growth of scientific publications \cite{fortunato2018science, bornmann2021growth, jinha2010article, van2014global} and the increasingly interdisciplinary nature of science \cite{van2015interdisciplinary, okamura2019interdisciplinarity}. However, current approaches such as using textual or visual search engines and reading survey papers are limited in terms of sensemaking support or timeliness. Scholarly search engines such as Google Scholar\footnote{\url{scholar.google.com}} and Semantic Scholar\footnote{\url{www.semanticscholar.org}} while effective in finding individual papers about a query, they do not show latent connections between papers to present an overview of the space \cite{marchionini2006exploratory, russell1993cost}. Contrastly, visualization tools, like Connected Papers\footnote{\url{www.connectedpapers.com}}, cluster multiple papers based on their citations or word embeddings. However, automatic clusters and complex graphs can be difficult for users to make sense of even after examining individual documents they often conflate multiple dimensions \cite{hearst2006clustering}. Therefore, scholars still need to examine individual papers to try to figure out the meaning of each automatically generated cluster and how different papers relate to one another \cite{chau2011apolo}. In contrast to these automated approaches    , topic survey papers present a broad overview of a research topic with coherent research themes and carefully synthesized descriptions \cite{bruce1994research, knopf2006doing}. However, since survey papers take significant manual effort to compile, they are not always available on all topics, and can quickly become outdated as new research emerges.


Meanwhile, authors already summarize prior work in papers’ related work sections when they publish a paper. For readers, related work sections of a paper could not only help better situate its contribution within the broader literature, it also allows scholars new to the domain to gain both a quick overview of the topic space and discover other prior work to further their readings \cite{tenopir2012article, teevan_2014}. However, the scope of a related work section is limited to supporting a single paper, and often not as comprehensive as a topic survey paper. In a formative study ($n=10$), we explored the potential for users to search and explore many related work section paragraphs extracted across multiple papers for a literature review task. We observed both benefits and challenges of reading multiple related work paragraphs discussing a complex scientific topic. We found that while this approach helped quickly explore different threads of research, scholars need help prioritizing and keeping track of related work paragraphs across papers that often overlap yet diverge in research foci and referenced literature (§\ref{sec:formative}). 

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{Images/RelatedlyPlain_v3.png}
\caption{The \textit{Relatedly} system user interface presents users with related work paragraphs from prior work discussing the topic, and scaffolds the topic exploration experience using features such as auto-generated descriptive paragraph titles,  dynamic re-ranking and highlighting to spotlight unseen dissimilar information, low-lighting of redundant text, and tracking information read}
\label{fig:Relatedly}
\end{figure} 

In this paper, we introduce a novel system, \textit{Relatedly}, to study a new approach for surveying literature where users are able to fluidly explore many related work sections extracted across multiple scholarly papers to gain a broad overview of an unfamiliar research area (Fig.~1). Given a query about a research topic, the system retrieves relevant paragraphs with their section headings to help users gain a quick overview of the different research threads. For example, when a user searched for ``misinformation'', from the section headings, they can quickly see different related work section paragraphs summarizing a wide range of research threads, including \emph{Automatic Fake News Detection}, \emph{Impact of Fake News on Public Opinion}, \emph{The Role of Journalists in Spreading and Correcting Misinformation} (Fig.~1). Since related work sections from different papers often cover overlapping topics and citations, \textit{Relatedly} provides information gain cues and progress tracking features to support reading them. For example, when reading a new paragraph, \textit{Relatedly} low-lights sentences about referenced papers that the user has explored in other paragraphs to avoid redundant effort. To help users quickly gain a broad overview of the information space, as a user explores the different paragraphs, \textit{Relatedly} keeps track of which paragraphs and references the user has explored to dynamically re-rank the remaining paragraphs and highlight unexplored references by estimating their novelty to the current user.

To evaluate this approach, we conducted a within-subjects study ($n=15$) where participants were asked to explore and make sense of scientific literature on two different multi-faceted exploratory topics, with the goal of outlining a survey paper on each topic, using \textit{Relatedly} for one topic and using the \textit{Baseline} system (similar to standard scholarly search where it is easy to read related work sections of papers) for the other. Analysis shows that when using the \textit{Relatedly} system, participants synthesized information better and produced better quality outlines when using the \textit{Relatedly} system, than when they were using the \textit{Baseline}. They also discovered significantly more papers, read more paragraphs across papers, and explored more diverse subtopics than when they were using \textit{Relatedly} rather than the \textit{Baseline} system. It also helped them discover more domain-specific terminology than \textit{Baseline}. When asked about which system they would prefer using for literature reviews, participants reported preferring to read related work sections using \textit{Relatedly} than a list of papers using the \textit{Baseline} system, particularly because it helped them understand relationships between concepts, prioritize what to read and keep track of information read during the literature review process. 

This work makes the following contributions: 
\begin{itemize}
    \item A novel approach to help scholars overview scientific topics by reading and exploring related work sections extracted across papers. We explore the unique user challenges of this approach in a formative user study with 10 participants.
    \item The \textit{Relatedly} system: which scaffolds this approach to discovering and systematically reviewing literature on a scientific topic with reading and prioritization support features such as low-lighting of redundant text, dynamic re-ranking and highlighting to spotlight unseen information, and auto-generated descriptive paragraph titles,
    \item Empirical insights from a within-subject study with 15 participants and the voluntary extended use of 5 participants that suggest presenting rich context and structure from prior related work sections with reading support and information gain tracking features promotes literature discovery and synthesis helping participants generate better learning summaries that are more coherent, insightful, and comprehensive. 
\end{itemize}



==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX
